How the level sampling process impacts zero-shot generalisation in deep reinforcement learning

A key limitation preventing the wider adoption of autonomous agents trained via deep reinforcement learning (RL) is their limited ability to generalise to new environments, even when these share similar characteristics with environments encountered during training. In this work, we investigate how a non-uniform sampling strategy of individual environment instances, or levels, affects the zero-shot generalisation (ZSG) ability of RL agents, considering two failure modes: overfitting and over-generalisation. As a first step, we measure the mutual information (MI) between the agent's internal representation and the set of training levels, which we find to be well-correlated to instance overfitting. In contrast to uniform sampling, adaptive sampling strategies prioritising levels based on their value loss are more effective at maintaining lower MI, which provides a novel theoretical justification for this class of techniques. We then turn our attention to unsupervised environment design (UED) methods, which adaptively generate new training levels and minimise MI more effectively than methods sampling from a fixed set. However, we find UED methods significantly shift the training distribution, resulting in over-generalisation and worse ZSG performance over the distribution of interest. To prevent both instance overfitting and over-generalisation, we introduce self-supervised environment design (SSED). SSED generates levels using a variational autoencoder, effectively reducing MI while minimising the shift with the distribution of interest, and leads to statistically significant improvements in ZSG over fixed-set level sampling strategies and UED methods.

==> obsolete.tex <==

\section{Preliminary draft}\label{sec:prog}
Lemmas from \cref{fig:lemmas_instance_based_gen} show that in the ZSG setting this gap is bounded by $\mut (\pi,L)$, the mutual information between any instance $i \in L$ and the learnt policy network, divided between the state belief function $b$ outputting the final representation layer of the policy network $b(H^o_t)=z_t$ (or $b(o_t)=z_t$ for non recurrent policies) and the policy head (\textit{they refer to the policy head as $\pi$ in \cref{fig:lemmas_instance_based_gen}, we refer to it as $g_\theta$ and use $\pi_\theta = b \circ g_\theta$ to avoid confusion in our notation}).

\begin{figure}[H]
    \centering
    \fbox{\includegraphics[width=1\linewidth]{iclr2023/content/instance_based_generalization_lemmas.png}}
    \caption{Lemmas of interest from \cite{instance_invariant}.}
    \label{fig:lemmas_instance_based_gen}
\end{figure}

\textit{Note: obtaining a generalization bound in the robust ZSG setting (independently of whether it is derived as a function of mutual information) would require some strong assumptions, such as regret smoothness over $C, \forall \pi \in \Pi$ and $|L|$ being large enough to contain a good approximation of its global minima. Convexity may also be required, as if there exist local minima there is no guarantee that a policy optimised to approach a local minima does not have an arbitrarily large regret when evaluated at the global regret minima of the joint $\Pi \times C$ space.  This makes the objective defined in \cref{eq:minimax_regret_empirical} questionable and, in my opinion this is a strong argument against employing a minimax regret game formulation whenever $C_\text{train} \subset C$. It may be worth it to investigate this more formally.}


We can optimise for \cref{eq:avg_return} by optimizing the empirical objective \cref{eq:avg_return_empirical} while at the same time minimising the generalization gap. We may minimise the gap by minimising its upper bound, i.e. by minimising $\mut (\pi,L)$. While prior work \citep{instance_invariant} %
achieves this by learning an ensemble of policies, we act on the sampling process of individual levels by controlling $p(i)$. We further make two modifications:
\begin{enumerate}
    \item By the data processing inequality, $\mut (b\circ g_\theta,L) \leq \mut (b, L)$, which means we can minimise $\mut (\pi,L)$ by minimising $\mut(Z,L)$, which treats the outputs of the penultimate layer of $\pi_\theta$ as the random variable $Z$.
    \item We sample levels from some finite subset $I$. We start by studying the case where $I=L$. To include frameworks sampling over the full level space, we also study the case where we have access to $L$ but $|L|=|X|$ (for example, a framework leveraging the provided training level set $L$ to learn a generative model over $X$).
\end{enumerate}

We now present our main theoretical results.

\begin{theorem} \label{th:mi_kld}
    Given a learned belief function such that $\vh = b (H_t^o)$, we can approximately minimize $\mut (L,b)$ by minimizing 
    \begin{equation}
         \mathcal{H}(p(i)) + \mathbb{E}_{(i, H_t^o) \in B} \log p(i|b (H_t^o)),
    \end{equation}
    where $B$ represents a batch of observations or histories collected by $\pi_\theta$.

    proof:

    \begin{align}\label{eq:proof_mi_kld}
        \mut(L,b) &= \sum_{i \in L} \int d\vh p(\vh,i) \log \frac{p(\vh,i)}{p(\vh)p(i)} \\
        &= - \sum_{i \in L} \int d\vh p(\vh,i) \log p(i) + \sum_{i \in L} \int d\vh p(\vh, i) \log p(i|\vh) \\
        &\approx \mathcal{H}(p(i)) + \frac{1}{|B|} \sum^{|B|}_{n} \log p(i^{(n)}|\vh^{(n)}) \label{eq:proof_empirical_approx}\\
        &= \mathcal{H}(p(i)) + \mathbb{E}_{(i, H_t^o)^{(n)} \in B} \log p(i|b (H_t^o))
    \end{align}


    where in \cref{eq:proof_empirical_approx} we approximate $p(\vh,i)$ as the empirical distribution

    \begin{equation} \label{eq:empirical_approx}
        \tilde{p}(\vh,i) = 
        \begin{cases}
            \frac{1}{|B|} &\text{ if } (H_t^o, i) \in B, \text{ with } \vh = b(H_t^o) \\
            0 &\text{ otherwise.}
        \end{cases}
    \end{equation}
    
\end{theorem}

Directly following \cref{th:mi_kld}, we have the lemma:

\begin{lemma} \label{lem:mi_h_crossh}
     We can approximately minimize $\mut (L,b)$ by minimizing 

    \begin{equation}
       \mathcal{H}(p(i)) + \frac{1}{|B|} \sum^{|L|}_j p(j) \sum^{|\tau_j|}_k \log p(j|b(H_k^o)),
    \end{equation}

    where $\tau_j$ represent the (or set of) trajectories from instance $j$ present in $B$.
\end{lemma}

Hence $\mut (L,b)$ is minimised by jointly minimising the entropy of $p(i)$ and maximising the cross-entropy between $p(i)$ and $p(i|\vh)$. It can be shown that if we set $p$ to the uniform distribution, increasing $|L|$ strictly minimises mutual information.
\textit{I have a proof but not included here, essentially we can show that while increasing the support size raises the entropy it increases the cross-entropy faster and overall the mutual information gets smaller. It is probably possible to show this for any distribution, not just the uniform one, but the proof is likely more involved}. %
This supports the intuitive notion that increasing the number of levels within the training set reduces the generalization gap. 

More surprisingly, when considering a finite number of instances it indicates that setting $p$ to the uniform distribution does not automatically minimize $\mut(L,b)$, and hints at the existence of adaptive distributions $p$ minimising $\mut(L,b)$ better than the uniform distribution, by specifically targeting the maximisation of the cross-entropy term.

\subsection{Instance information minimisation when $I = L$}

This is the setting where we are limited to sampling training levels from $L$ (i.e. the \textit{controllable} level space $I = L$). In order to compute $\mut (L,b)$, we need to model $p(i|\vh)$. If $X$ is limited to a finite and small set of seeds, such as in the ProcGen benchmark \citep{procgen}, our best course of action to treat each seed as a separate label and learn a classifier computing $p(i|\vh)$.

\subsection{Instance information minimisation when $I\supset L$ and $|L| = |X|$}

Below are the main points to make in the write-up.

\begin{enumerate}

    \item An effective way of minimising $\mut (L,b)$ is to increase $|L|$, therefore if we have access to the full level space it is beneficial to utilise it.
    \item In settings where an instance is not represented implicitly as a random seed or one-hot vector but explicitly as a vector of environment parameters $\rvx$, it would be useful to exploit the information in $\rvx$ instead of simply treating each level as a label.
    \item This is where we could explore how we can make use of our beta-VAE model, which models the generative process $\tilde{C} \rightarrow X$, where $\tilde{\vc}$ is a latent vector representing the underlying factors of variations in $X$, and may be viewed as a minimal representation for the context. We can make use of the generative model to augment $I$ to include in-context synthetic levels. This is useful if the context space maps to a small subset of $X$ (for example level spaces with many unsolvable levels), or in level spaces where multiple CMDP exist and have conflicting optimal policies. \textit{This is where we can plug some of our existing results in.}
    \item In making the VAE a part of the instance generation pipeline, we change the data generation Markov chain $I\rightarrow \tau \leftarrow \pi$ to $I\rightarrow X \rightarrow \tilde{C} \rightarrow \tilde{X} \rightarrow \tilde{I} \rightarrow \tau \leftarrow \pi$.  \cite{VIB} show that given data $X$ and latent space $\tilde{C}$ the beta VAE's variational objective maximises $\mut (X,\tilde{C}) - \beta \mut(i, \tilde{C})$ or in other words maximises the information contained in the input data while minimising the information shared with any individual instance. This places an information bottleneck in our data generation pipeline and, by the data processing inequality it minimises $\mut (I, \pi)$.
    \item It is possible to further minimise $\mut (I, \pi)$ by placing another information bottleneck on $\mut (I, Z)$ through controlling the level sampling process. Given a training dataset $L$, we employ $K\leq|L|$ \textit{level instantiating processes}, where each process can instantiate multiple synthetic instances from $\tilde{I}$. We sample instances $\tilde{i}$ such that they minimise $p(k|{\vh}_{\tilde{i}})$, i.e. the probability of being in instance generating process $k$ given the latent representations obtained from synthetic instance $\tilde{i}$. \textit{(I have not typed in the proof yet but it can be shown that we can recover a formulation for $p(k|{\vh}_{\tilde{i}})$ using the VAE, while we can modulate $K$ so that it remains feasible to learn a discrete classifier.)}
    \item We are conditioning the level instantiating processes on levels $L$ collected from the underlying context distribution, and we sample uniformly from $K$ when selecting an instance generating process. We minimise  $\mut (I, Z)$ through controlling $p(\tilde{i}|k)$ (i.e. the probability of sampling a given synthetic level from instance generating process $k$). By doing so we stay close to the underlying context distribution and we mitigate covariate-shift issues induced by PLR, a limitation of this class of techniques first reported in \cite{SAMPLR}. \textit{(To show this, we use the VAE's capability of being able to sample $\tilde{\rvx}$ conditioned on some sample $\rvx_i$. If we perform this sampling process with ${\rvx}_i \sim p(\rvx)$ then any of the resulting synthetic $\tilde{X}$ are sampled from the variational approximation $\tilde{p}(\rvx)$}.
    \item An area of future work would be to explore other variational models (for example the CVAE \citep{CVAE}, a diffusion model, or a joint learning technique) to measure $\mut (L,b)$, by modelling (implicitly or explicitly) $p(i|\vh)$ as before and/or other formulations of the mutual information relying on $p(\vh|i)$ or $p(i,\vh)$.

\end{enumerate}


\subsection{ZSG as an asymmetric minimax mutual information game.}
\textit{Note: not sure this section has its place in this paper, curious to hear your opinion on this.}

\begin{theorem} \label{th:actor_critic_mi}
   In a single instance MDP, Minimising the actor critic loss
\begin{equation}
    L_{AC} = - J^{\pi}_{PG} + \alpha L_V,
\end{equation}
where $J^{PG}_\pi$ is the policy gradient objective, $L_V$ is the  $\ell_2$ value loss and $\alpha$ is a scaling hyperparamter may be reformulated as maximising the information maximisation objective
\begin{equation}
    \mut(Z, A^*) + \alpha \mut(Z,V).
\end{equation}

draft proof: It can be shown that
\begin{enumerate}
    \item Minimising the $\ell_2$ value loss is equivalent to maximising $\mut(Z,V)$. The derivation is trivial, simply linear regression with the modelling assumption that $V^\pi= h_\theta(\vh) + \epsilon, \epsilon \sim \mathcal{N}(0,1)$ and $h_\theta$ being the critic head.
    \item Maximising the policy gradient objective is equivalent to maximising $\mut(Z, A^*)$, $A^*$ being the random variable representing the output of the optimal policy of the MDP. Not sure how to write a complete proof but the sketch for it would be as follows and borrows from arguments made in \cite{vib_actor_critic}: 
    \begin{enumerate}
       \item Maximising $\mut(Z, A^\pi)$ is equivalent to maximising $\mathbb{E}_{s\sim\rho{^\pi}(s)}[\log p(a|b(s))]=\mathbb{E}_{s\sim\rho{^\pi}(s)}[\log (b(s) \circ g_\theta)]=\mathbb{E}_{s\sim\rho{^\pi}(s)}[\log \pi_\theta(s)]$
        \item The PG objective maximises $\mathbb{E}_{s\sim\rho{^\pi}(s), a\sim \pi_\theta(s)}[\log \pi_\theta(s)\text{Adv}^{\pi}(a,s)]$, where $\text{Adv}^\pi$ is the advantage function. Then under an argument of convergence of the PG theorem to the optimal policy we could prove that we converge to maximising $\mathbb{E}_{s\sim\rho{^\pi}(s)}[\log p(a^*|b(s))]$ and therefore maximising $\mut(Z, A^*)$
    \end{enumerate}

\end{enumerate} 
\end{theorem}

In a CMDP we must also minimise $\mut(Z, I)$ to avoid overfitting to specific instances. We must therefore modify our objective to include an information bottleneck
\begin{equation}
    \max \mut(Z, A^*) + \alpha \mut(Z,V) - \beta \mut(Z, I),
\end{equation}
where $\beta$ is a scaling parameter. Existing work on generalizable state representations can be reframed under this lens (e.g. \cite{MICo, PSM}. However, as shown by \cref{th:mi_kld} we can minimise $\mut(Z, I)$ separately through $p(i)$. Doing so is akin to playing an asymmetric mutual information game between the agent and the task sampler. The agent's objective is to maximise $\mut(Z, A^*) + \alpha \mut(Z,V)$, which is equivalent to applying the standard actor-critic objective, as demonstrated in \cref{th:actor_critic_mi}. The task sampler objective is to pick $p(i)$ satisfying
\begin{equation}
    \argmin_{p(i)} \mut(Z, I)
\end{equation}
which we can optimise using results from \cref{th:mi_kld}.



